DynaPrompt: Dynamic Test-Time Prompt Tuning

Test-time prompt tuning enhances zero-shot generalization of vision-language models but tends to ignore the relatedness among test samples during inference. Online test-time prompt tuning provides a simple way to leverage the information in previous test samples, albeit with the risk of prompt collapse due to error accumulation. To enhance test-time prompt tuning, we propose DynaPrompt, short for dynamic test-time prompt tuning, exploiting relevant data distribution information while reducing error accumulation. Built on an online prompt buffer, DynaPrompt adaptively selects and optimizes the relevant prompts for each test sample during tuning. Specifically, we introduce a dynamic prompt selection strategy based on two metrics: prediction entropy and probability difference. For unseen test data information, we develop dynamic prompt appending, which allows the buffer to append new prompts and delete the inactive ones. By doing so, the prompts are optimized to exploit beneficial information on specific test data, while alleviating error accumulation. Experiments on fourteen datasets demonstrate the effectiveness of dynamic test-time prompt tuning.

==> figures/ablation.tex <==
\begin{figure}[t]
    \centering
    \begin{minipage}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/ablations/num_p_a1.png}
        \subcaption{Top-1 Accuracy of different prompt buffer sizes.}
        \label{fig:nump}
    \end{minipage}
    \hfill
    \begin{minipage}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/ablations/timecost1.png}
        \subcaption{Time costs with different prompt buffer sizes.}
        \label{fig:timecost}
    \end{minipage}
    \hfill
    \begin{minipage}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/ablations/samo_a.png}
        \subcaption{Different sample orders for ImageNet-A.}
        \label{fig:order_a}
    \end{minipage}
    \hfill
    \begin{minipage}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/ablations/samo_r.png}
        \subcaption{Different sample orders for ImageNet-R.}
        \label{fig:order_r}
    \end{minipage}
    \vspace{-2mm}
    \caption{\textbf{Influence of the prompt buffer size on performance (a) and time costs (b), as well as the sensitivity on the online sample orders on ImageNet-A (c) and ImageNet-R (d).} Larger buffer sizes lead to better performance with higher costs. The online sample order slightly affects performance, especially with fewer samples (c).}
    \label{fig:overall_figure}
    \vspace{-4mm}
\end{figure}

==> tables/crossdataset0.tex <==
\begin{table*}[t]
\begin{center}
% \vspace{-2mm}
	\resizebox{1\columnwidth}{!}{%
		% \setlength\tabcolsep{4pt} 
\begin{tabular}{lccccccccccc}
\toprule
% & \multicolumn{4}{c}{Domain Generalization datasets} & \multicolumn{4}{c}{ImageNet-based covariate shift} \\ 
% \cmidrule(lr){2-5} \cmidrule(lr){6-9}
% Caltech 	Pets 	Cars 	Flowers 	Food101 	Aircraft 	SUN397 	DTD 	EuroSAT	UCF101 	Average
 Method  & \rot{Caltech} & \rot{Pets} & \rot{Cars} & \rot{Flowers} &\rot{Food101} &\rot{Aircraft} &\rot{SUN397} &\rot{DTD} &\rot{EuroSAT} &\rot{UCF101} & \rot{\textit{Mean}} \\ \midrule
 % \rowcolor{mColor1}
% CLIP \citep{radford2021learning} & 93.35 & 88.25 & 65.48 & 67.44 & 83.65 & 23.67 & 62.59 & 44.27 & 42.01 & 65.13 & 63.58 \\
% TPT + CLIP \citep{shu2022test}  & 94.16 & 87.79 & 66.87 & 68.98 & 84.67 & \textbf{24.78} & 65.50 & 47.75 & \textbf{42.44} & 68.04 & 65.10 \\
CLIP & 93.35 & 88.25 & 65.48 & 67.44 & 83.65 & 23.67 & 62.59 & 44.27 & 42.01 & 65.13 & 63.58 \\
TPT + CLIP  & 94.16 & 87.79 & 66.87 & 68.98 & 84.67 & \textbf{24.78} & 65.50 & 47.75 & \textbf{42.44} & 68.04 & 65.10 \\
\rowcolor{lightblue}
\textit{\textbf{This paper}} + CLIP & \textbf{94.32} & \textbf{88.28} & \textbf{67.65} & \textbf{69.95} & \textbf{85.42} & {24.33} & \textbf{66.32} & \textbf{47.96} & {42.28} & \textbf{68.72} & \textbf{65.52} \\
\midrule
% CoOp \citep{zhou2022learning} & {64.20} & 47.99 & 49.71 & 75.21 & 59.28 & & & & & & \\
% TPT + CoOp \citep{shu2022test} & {66.83} & 49.29 & 57.95 & 77.27 & 62.84 & & & & & & \\
% \rowcolor{lightblue}
% \textit{\textbf{This paper}} + CoOp & & & & & & & & & & & \\
% \midrule
% % CoCoOp \cite{zhou2022conditional} & 64.07 & {48.75} & {50.63} & {76.18}  \\
% % TPT + CoCoOp \cite{shu2022test}  & 64.85 & 48.47 & {58.47}  & 78.65 \\
% % This paper + CoOp & & & & \\
% %\rowcolor{Gray}
% 93.53 90.49 65.57 72.23 86.20 24.74 67.01 46.49 48.06  
% MaPLe \citep{khattak2023maple} & 93.53 & 90.49 & 65.57 & 72.23 & 86.20 & 24.74 & 67.01 & 46.49 & \textbf{48.06} & 68.69 & 66.30 \\
% TPT + MaPLe \citep{shu2022test} & 93.59 & 90.72 & 66.50 & 72.37 & 86.64 & 24.70 & 67.54 & 45.87 & 47.80 & 69.19 & 66.49 \\
% PromptAlign \citep{samadh2023align} & 94.01 & 90.76 & \textbf{68.50} & 72.39 & \textbf{86.65} & \textbf{24.80} & 67.54 & 47.24 & {47.86} & 69.47 & 66.92 \\
MaPLe & 93.53 & 90.49 & 65.57 & 72.23 & 86.20 & 24.74 & 67.01 & 46.49 & \textbf{48.06} & 68.69 & 66.30 \\
TPT + MaPLe & 93.59 & 90.72 & 66.50 & 72.37 & 86.64 & 24.70 & 67.54 & 45.87 & 47.80 & 69.19 & 66.49 \\
PromptAlign & 94.01 & 90.76 & \textbf{68.50} & 72.39 & \textbf{86.65} & \textbf{24.80} & 67.54 & 47.24 & {47.86} & 69.47 & 66.92 \\
\rowcolor{lightblue}
\textit{\textbf{This paper}} + MaPLe & \textbf{95.17} & \textbf{90.95} & {68.26} & \textbf{73.28} & {86.60} & 24.36 & \textbf{68.18} & \textbf{48.75} & 47.53 & \textbf{69.85} & \textbf{67.29} \\
\bottomrule
% 95.17	90.95									
\end{tabular}
}
\end{center}
% \vspace{-6mm}
\caption{\textbf{Comparisons on the cross-dataset setting.}
}
\label{tab:cd}
% \vspace{-6mm}
\end{table*}

==> tables/domain.tex <==
\begin{table*}[t]
\caption{\textbf{Comparisons on the domain generalization setting} with both prompt learning and test-time prompt tuning methods.
The prompt learning methods train their prompts on ImageNet.
The proposed method outperforms both kinds of methods in terms of Top-1 accuracy. Combining our method with pretrained prompts further improves the performance. 
% \cs{Why not report This paper + PromptAlign? I don't see much benefit to report This paper + MaPLe, we outperform it for most datasets with This paper + CoOp.}
}
\label{tab:dg}
\vspace{-2mm}
\begin{center}
% \vspace{-2mm}
	\resizebox{0.98\columnwidth}{!}{%
		% \setlength\tabcolsep{4pt} 
\begin{tabular}{l lllll}
\toprule
% & \multicolumn{4}{c}{Domain Generalization datasets} & \multicolumn{4}{c}{ImageNet-based covariate shift} \\ 
% \cmidrule(lr){2-5} \cmidrule(lr){6-9}
Method  & {ImageNet-V2} & {ImageNet-S} & {ImageNet-A} & {ImageNet-R} & \textit{Mean} \\ \midrule
 CLIP \citep{radford2021learning} & 60.83 & 46.15 & 47.77 & 73.96 & 57.23 \\
\midrule
\rowcolor{mColor1}
\multicolumn{6}{c}{Prompt learning methods without test-time tuning} \\
CoOp \citep{zhou2022learning} & {64.20} & 47.99 & 49.71 & 75.21 & 59.28 \\
CoCoOp \citep{zhou2022conditional} & 64.07 & 48.75 & 50.63 & 76.18 & 59.90 \\
KgCoOp \citep{yao2023visual} & 64.10 & 48.97 & 50.69 & 76.70 & 60.11 \\
MaPLe \citep{khattak2023maple} & 64.07 & 49.15 & 50.90 & 76.98 & 60.28 \\
CoPrompt \citep{roy2024consistency} & 64.25 & 49.43 & 50.50 & 77.51 & 60.42 \\
Any-shift Prompt \citep{xiao2024any} & {64.53} & {49.80} & {51.52} & {77.56} & 60.85 \\
\midrule
\rowcolor{mColor1}
\multicolumn{6}{c}{Test-time prompt tuning methods} \\
TPT \citep{shu2022test}  & 63.45 & 47.94 & {54.77} & 77.06 & 60.81 \\
DiffTPT \citep{feng2023diverse} & 65.10  & 46.80 & 55.68 & 75.00 & 60.65 \\
C-TPT \citep{yoon2024c} & 63.40 & 48.50 & 52.90 & 78.00 & 60.70 \\
\rowcolor{lightblue}
\textit{\textbf{This paper}} & {64.67} & {48.22} & {56.17} & {78.17} & {61.81} \\
\midrule
CoOp + TPT \citep{shu2022test} & {66.83} & 49.29 & 57.95 & 77.27 & 62.84 \\
\rowcolor{lightblue}
CoOp + \textit{\textbf{This paper}} & \textbf{67.25} & \textbf{50.28} & 60.55 & 79.15 & \textbf{64.31} \\
\midrule
% CoCoOp \cite{zhou2022conditional} & 64.07 & {48.75} & {50.63} & {76.18}  \\
% TPT + CoCoOp \cite{shu2022test}  & 64.85 & 48.47 & {58.47}  & 78.65 \\
% This paper + CoOp & & & & \\
%\rowcolor{Gray}
MaPLe + TPT \citep{shu2022test} & 64.87 & 48.16 & 58.08 & 78.12 & 62.31 \\
MaPLe + PromptAlign \citep{samadh2023align} & 65.29 & 50.23 & 59.37 & 79.33 & 63.56 \\
\rowcolor{lightblue}
MaPLe + \textit{\textbf{This paper}} & {66.34} & {50.25} & \textbf{60.72} & \textbf{79.57} & {64.22} \\
\bottomrule
\end{tabular}
}
\end{center}
\vspace{-2mm}
\end{table*}

==> tables/selection_metrics.tex <==
\begin{table*}[t]
\caption{\textbf{Ablations on dynamic prompt selection metrics.} Either without the entropy or the confidence selection metrics leads to obvious performance degradation.
}
\label{tab:strategy}
\vspace{-4mm}
\begin{center}
% \vspace{-2mm}
	\resizebox{1\columnwidth}{!}{%
		% \setlength\tabcolsep{4pt} 
\begin{tabular}{l ccccc}
\toprule
% & \multicolumn{4}{c}{Domain Generalization datasets} & \multicolumn{4}{c}{ImageNet-based covariate shift} \\ 
% \cmidrule(lr){2-5} \cmidrule(lr){6-9}
Method  & {ImageNet-V2} & {ImageNet-S} & {ImageNet-A} & {ImageNet-R} & \textit{Mean} \\ \midrule
 % CLIP \citep{radford2021learning} & 60.83 & 46.15 & 47.77 & 73.96 & 57.23 \\
% \midrule
% \rowcolor{mColor1}
% \multicolumn{6}{c}{Dynamic prompt selection strategy} \\
w/o entropy & 61.45 & 46.86 & 50.25 & 76.19 &  58.69 \\
w/o confidence & 61.93 & 46.95 & 50.95 & 77.37 &  59.23 \\
% 61.45	46.86	50.25	76.19	58.6875
% 61.93	46.95	50.95	77.37	59.225
% 64.67	48.22	56.17	78.17	56.35333333
% \midrule
% \rowcolor{mColor1}
% \multicolumn{6}{c}{Dynamic prompt appending strategy} \\
% w/o dynamic appending &  &  & 30.74 &  & \\
% \midrule
With both selection metrics & {64.67} & {48.22} & {56.17} & {78.17} & {61.81} \\
\bottomrule
\end{tabular}
}
\end{center}
\vspace{-4mm}
\end{table*}


\begin{table*}[t]
\caption{\textbf{Ablations on dynamic prompt appending strategy.} Without the appending strategy, the performance drops considerably due to error accumulation and prompt collapse. \cs{suggest to group Table 3 and 4 on the same page, more convenient for the reader.}
}
\label{tab:appstrategy}
\vspace{-2mm}
\begin{center}
% \vspace{-2mm}
	\resizebox{1\columnwidth}{!}{%
		% \setlength\tabcolsep{4pt} 
\begin{tabular}{l ccccc}
\toprule
% & \multicolumn{4}{c}{Domain Generalization datasets} & \multicolumn{4}{c}{ImageNet-based covariate shift} \\ 
% \cmidrule(lr){2-5} \cmidrule(lr){6-9}
Method  & {ImageNet-V2} & {ImageNet-S} & {ImageNet-A} & {ImageNet-R} & \textit{Mean} \\ \midrule
 % CLIP \citep{radford2021learning} & 60.83 & 46.15 & 47.77 & 73.96 & 57.23 \\
% \midrule
% \rowcolor{mColor1}
% \multicolumn{6}{c}{Dynamic prompt selection strategy} \\
% Dynamic selection w/o entropy &  &  & 50.25 &  &  \\
% Dynamic selection w/o APD &  & & 50.95 &  &  \\
% \midrule
% \rowcolor{mColor1}
% \multicolumn{6}{c}{Dynamic prompt appending strategy} \\
w/o dynamic appending & 35.66 & 20.38 & 30.74 & 43.72 & 32.63 \\
% \midrule
w/ dynamic appending & {64.67} & {48.22} & {56.17} & {78.17} & {61.81} \\
\bottomrule
\end{tabular}
}
\end{center}
\vspace{-2mm}
\end{table*}
